Using Taylor-Approximated Gradients to Improve the Frank-Wolfe Method for Empirical Risk Minimization

The Frank-Wolfe method has become increasingly useful in statistical and machine learning applications, due to the structure-inducing properties of the iterates, and especially in settings where linear minimization over the feasible set is more computationally efficient than projection. In the setting of Empirical Risk Minimization -- one of the fundamental optimization problems in statistical and machine learning -- the computational effectiveness of Frank-Wolfe methods typically grows linearly in the number of data observations $n$. This is in stark contrast to the case for typical stochastic projection methods. In order to reduce this dependence on $n$, we look to second-order smoothness of typical smooth loss functions (least squares loss and logistic loss, for example) and we propose amending the Frank-Wolfe method with Taylor series-approximated gradients, including variants for both deterministic and stochastic settings. Compared with current state-of-the-art methods in the regime where the optimality tolerance $\varepsilon$ is sufficiently small, our methods are able to simultaneously reduce the dependence on large $n$ while obtaining optimal convergence rates of Frank-Wolfe methods, in both the convex and non-convex settings. We also propose a novel adaptive step-size approach for which we have computational guarantees. Last of all, we present computational experiments which show that our methods exhibit very significant speed-ups over existing methods on real-world datasets for both convex and non-convex binary classification problems.

==> preamble2.tex <==
\usepackage[mathscr]{eucal}
%\usepackage[cmex10]{amsmath}
\usepackage{epsfig,epsf,psfrag}
\usepackage{amssymb,amsmath,amsfonts,latexsym}
\usepackage{graphicx}
%\usepackage{epstopdf}
\usepackage{epstopdf}
\usepackage{bm,xcolor,url}
\usepackage[caption=false]{subfig} 
\usepackage{fixltx2e}%ordering of single and double column floats
\usepackage{array}%array and tabular environments
\usepackage{verbatim}
\usepackage{bm}
\usepackage{algpseudocode, cite}
\usepackage{algorithm}
\usepackage{verbatim}
\usepackage{textcomp}
\usepackage{mathrsfs}
%\usepackage{ntheorem}
%\usepackage{hyperref}
%\usepackage{epstopdf}
%\usepackage{setspace}
\usepackage{relsize}
%\usepackage{cleveref} 
\usepackage{subfig}
\usepackage{amsthm}
\usepackage{enumerate}
%\usepackage{subfigure}
%\usepackage{subcaption}
%\usepackage{url}
\usepackage{setspace}
\usepackage{cases}
\usepackage{footnote}
\usepackage{tabularx,tabu}
\usepackage{tablefootnote}
\usepackage{threeparttable}
\usepackage{tikz}
\usetikzlibrary{datavisualization}
\usetikzlibrary{datavisualization.formats.functions}
\usetikzlibrary{decorations.pathreplacing}
\usepackage{textcomp}
\usepackage{multicol}
\usepackage{lipsum}
%\usepackage{bold-extra}
%\usepackage{beramono}
%\usepackage{lmodern}
%\newcommand{\span}{\mathrm{span}}
 
%% To produce a tilde in url
\catcode`~=11 \def\UrlSpecials{\do\~{\kern -.15em\lower .7ex\hbox{~}\kern .04em}} \catcode`~=13 

\allowdisplaybreaks[3]

\newcommand{\calHN}{\calH\calN} 
\newcommand{\iidsim}{\widesim{iid}}
\newcommand{\vecz}{\mathbf{0}}
\newcommand{\vecone}{\mathbf{1}}
\newcommand{\Iff}{if and only if\;\,} 
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\normt}[1]{\Vert#1\Vert}
\newcommand{\abst}[1]{\left\vert#1\right\vert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\lrpar}[1]{\left(#1\right)}
\newcommand{\lrang}[1]{\left\langle#1\right\rangle}
\newcommand{\lrbrace}[1]{\left\{#1\right\}}
\newcommand{\as}{{\rm \;\;a.s.}}
\newcommand{\nn}{\nonumber} 
\newcommand{\cequal}{\stackrel{\mathrm{c}}{=}}
\newcommand{\dequal}{\stackrel{\mathrm{d}}{=}}
\newcommand{\St}{\mathrm{subject\; to}}
%\newcommand{\defeq}{\stackrel{\scriptscriptstyle\Delta}{=}}
\newcommand{\defeq}{\triangleq}
\newcommand{\eqcst}{\stackrel{{\rm c}}{=}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}} 
\newcommand{\prox}{\mathbf{prox}}
\newcommand{\dom}{\mathbf{dom}}
\newcommand{\wrt}{w.r.t.\,}
\newcommand{\tilell}{\widetilde{\ell}}
\newcommand{\widesim}[2][1.5]{\mathrel{\overset{#2}{\scalebox{#1}[1]{$\sim$}}}}
\newcommand{\convu}{\xrightarrow{{\rm u}}}
\newcommand{\inter}{\mathbf{int}\,}
\newcommand{\bdr}{\mathbf{bd}\,}
\newcommand{\cl}{\mathbf{cl}\,}
\newcommand{\conv}{\mathbf{conv}\,}
\newcommand{\convcl}{\overline{\mathbf{conv}\,}}
\newcommand{\convinf}[1]{\xrightarrow{#1\to\infty}}
\newcommand{\diam}{\mathbf{diam}\,}
\newcommand{\dist}{\mathbf{dist}\,}
\newcommand{\hpartial}{\hat{\partial}}
\newcommand{\scHN}{\mathscr{H\hspace{-.15cm}N\hspace{-0cm}}}
\newcommand{\snr}{\mathtt{SNR}}
%\newcommand{\scSt}{\mathscr{St}}
\newcommand{\Section}[1]{\vspace{-8pt}\section{\hskip 0em~~#1}\vspace{-1pt}}
\newcommand{\Subsection}[1]{\vspace{-8pt}\subsection{\hskip -1em~~#1}\vspace{-3pt}}
\newcommand{\eps}{\epsilon}
\font\btt=rm-lmtk10

%Bold bar
\newcommand{\barba}{\overline{\bf{a}}}
\newcommand{\barbb}{\overline{\bf b}}
\newcommand{\barbc}{\overline{\bf c}}
\newcommand{\barbd}{\overline{\bf d}}
\newcommand{\barbe}{\overline{\bf e}}
\newcommand{\barbf}{\overline{\bf f}}
\newcommand{\barbg}{\overline{\bf g}}
\newcommand{\barbh}{\overline{\bf h}}
\newcommand{\barbi}{\overline{\bf i}}
\newcommand{\barbj}{\overline{\bf j}}
\newcommand{\barbk}{\overline{\bf k}}
\newcommand{\barbl}{\overline{\bf l}}
\newcommand{\barbm}{\overline{\bf m}}
\newcommand{\barbn}{\overline{\bf n}}
\newcommand{\barbo}{\overline{\bf o}}
\newcommand{\barbp}{\overline{\bf p}}
\newcommand{\barbq}{\overline{\bf q}}
\newcommand{\barbr}{\overline{\bf r}}
\newcommand{\barbs}{\overline{\bf s}}
\newcommand{\barbt}{\overline{\bf t}}
\newcommand{\barbu}{\overline{\bf u}}
\newcommand{\barbv}{\overline{\bf v}}
\newcommand{\barbw}{\overline{\bf w}}
\newcommand{\barbx}{\overline{\bf x}}
\newcommand{\barby}{\overline{\bf y}}
\newcommand{\barbz}{\overline{\bf z}}

\newcommand{\barbA}{\overline{\bf A}}
\newcommand{\barbB}{\overline{\bf B}}
\newcommand{\barbC}{\overline{\bf C}}
\newcommand{\barbD}{\overline{\bf D}}
\newcommand{\barbE}{\overline{\bf E}}
\newcommand{\barbF}{\overline{\bf F}}
\newcommand{\barbG}{\overline{\bf G}}
\newcommand{\barbH}{\overline{\bf H}}
\newcommand{\barbI}{\overline{\bf I}}
\newcommand{\barbJ}{\overline{\bf J}}
\newcommand{\barbK}{\overline{\bf K}}
\newcommand{\barbL}{\overline{\bf L}}
\newcommand{\barbM}{\overline{\bf M}}
\newcommand{\barbN}{\overline{\bf N}}
\newcommand{\barbO}{\overline{\bf O}}
\newcommand{\barbP}{\overline{\bf P}}
\newcommand{\barbQ}{\overline{\bf Q}}
\newcommand{\barbR}{\overline{\bf R}}
\newcommand{\barbS}{\overline{\bf S}}
\newcommand{\barbT}{\overline{\bf T}}
\newcommand{\barbU}{\overline{\bf U}}
\newcommand{\barbV}{\overline{\bf V}}
\newcommand{\barbW}{\overline{\bf W}}
\newcommand{\barbX}{\overline{\bf X}}
\newcommand{\barbY}{\overline{\bf Y}}
\newcommand{\barbZ}{\overline{\bf Z}}

\newcommand{\barell}{\overline{\ell}}
\newcommand{\barkappa}{\overline{\kappa}}

% Calligraphic stuff
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

\newcommand{\hatcalA}{\widehat{\calA}} 
\newcommand{\hatcalB}{\widehat{\calB}} 
\newcommand{\hatcalC}{\widehat{\calC}} 
\newcommand{\hatcalD}{\widehat{\calD}} 
\newcommand{\hatcalE}{\widehat{\calE}} 
\newcommand{\hatcalF}{\widehat{\calF}} 
\newcommand{\hatcalG}{\widehat{\calG}} 
\newcommand{\hatcalH}{\widehat{\calH}} 
\newcommand{\hatcalI}{\widehat{\calI}} 
\newcommand{\hatcalJ}{\widehat{\calJ}} 
\newcommand{\hatcalK}{\widehat{\calK}} 
\newcommand{\hatcalL}{\widehat{\calL}} 
\newcommand{\hatcalM}{\widehat{\calM}} 
\newcommand{\hatcalN}{\widehat{\calN}} 
\newcommand{\hatcalO}{\widehat{\calO}} 
\newcommand{\hatcalP}{\widehat{\calP}} 
\newcommand{\hatcalQ}{\widehat{\calQ}} 
\newcommand{\hatcalR}{\widehat{\calR}} 
\newcommand{\hatcalS}{\widehat{\calS}} 
\newcommand{\hatcalT}{\widehat{\calT}} 
\newcommand{\hatcalU}{\widehat{\calU}} 
\newcommand{\hatcalV}{\widehat{\calV}} 
\newcommand{\hatcalW}{\widehat{\calW}} 
\newcommand{\hatcalX}{\widehat{\calX}} 
\newcommand{\hatcalY}{\widehat{\calY}} 
\newcommand{\hatcalZ}{\widehat{\calZ}} 

\newcommand{\tilcalA}{\widetilde{\calA}} 
\newcommand{\tilcalB}{\widetilde{\calB}} 
\newcommand{\tilcalC}{\widetilde{\calC}} 
\newcommand{\tilcalD}{\widetilde{\calD}} 
\newcommand{\tilcalE}{\widetilde{\calE}} 
\newcommand{\tilcalF}{\widetilde{\calF}} 
\newcommand{\tilcalG}{\widetilde{\calG}} 
\newcommand{\tilcalH}{\widetilde{\calH}} 
\newcommand{\tilcalI}{\widetilde{\calI}} 
\newcommand{\tilcalJ}{\widetilde{\calJ}} 
\newcommand{\tilcalK}{\widetilde{\calK}} 
\newcommand{\tilcalL}{\widetilde{\calL}} 
\newcommand{\tilcalM}{\widetilde{\calM}} 
\newcommand{\tilcalN}{\widetilde{\calN}} 
\newcommand{\tilcalO}{\widetilde{\calO}} 
\newcommand{\tilcalP}{\widetilde{\calP}} 
\newcommand{\tilcalQ}{\widetilde{\calQ}} 
\newcommand{\tilcalR}{\widetilde{\calR}} 
\newcommand{\tilcalS}{\widetilde{\calS}} 
\newcommand{\tilcalT}{\widetilde{\calT}} 
\newcommand{\tilcalU}{\widetilde{\calU}} 
\newcommand{\tilcalV}{\widetilde{\calV}} 
\newcommand{\tilcalW}{\widetilde{\calW}} 
\newcommand{\tilcalX}{\widetilde{\calX}} 
\newcommand{\tilcalY}{\widetilde{\calY}} 
\newcommand{\tilcalZ}{\widetilde{\calZ}} 

\newcommand{\barcalA}{\overline{\calA}} 
\newcommand{\barcalB}{\overline{\calB}} 
\newcommand{\barcalC}{\overline{\calC}} 
\newcommand{\barcalD}{\overline{\calD}} 
\newcommand{\barcalE}{\overline{\calE}} 
\newcommand{\barcalF}{\overline{\calF}} 
\newcommand{\barcalG}{\overline{\calG}} 
\newcommand{\barcalH}{\overline{\calH}} 
\newcommand{\barcalI}{\overline{\calI}} 
\newcommand{\barcalJ}{\overline{\calJ}} 
\newcommand{\barcalK}{\overline{\calK}} 
\newcommand{\barcalL}{\overline{\calL}} 
\newcommand{\barcalM}{\overline{\calM}} 
\newcommand{\barcalN}{\overline{\calN}} 
\newcommand{\barcalO}{\overline{\calO}} 
\newcommand{\barcalP}{\overline{\calP}} 
\newcommand{\barcalQ}{\overline{\calQ}} 
\newcommand{\barcalR}{\overline{\calR}} 
\newcommand{\barcalS}{\overline{\calS}} 
\newcommand{\barcalT}{\overline{\calT}} 
\newcommand{\barcalU}{\overline{\calU}} 
\newcommand{\barcalV}{\overline{\calV}} 
\newcommand{\barcalW}{\overline{\calW}} 
\newcommand{\barcalX}{\overline{\calX}} 
\newcommand{\barcalY}{\overline{\calY}} 
\newcommand{\barcalZ}{\overline{\calZ}} 

% Boldface stuff
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\boldf}{\mathbf{f}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\boldm}{\mathbf{m}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bZ}{\mathbf{Z}}

% Roman stuff
\newcommand{\rma}{\mathrm{a}}
\newcommand{\rmA}{\mathrm{A}}
\newcommand{\rmb}{\mathrm{b}}
\newcommand{\rmB}{\mathrm{B}}
\newcommand{\rmc}{\mathrm{c}}
\newcommand{\rmC}{\mathrm{C}}
\newcommand{\rmd}{\mathrm{d}}
\newcommand{\rmD}{\mathrm{D}}
\newcommand{\rme}{\mathrm{e}}
\newcommand{\rmE}{\mathrm{E}}
\newcommand{\rmf}{\mathrm{f}}
\newcommand{\rmF}{\mathrm{F}}
\newcommand{\rmg}{\mathrm{g}}
\newcommand{\rmG}{\mathrm{G}}
\newcommand{\rmh}{\mathrm{h}}
\newcommand{\rmH}{\mathrm{H}}
\newcommand{\rmi}{\mathrm{i}}
\newcommand{\rmI}{\mathrm{I}}
\newcommand{\rmj}{\mathrm{j}}
\newcommand{\rmJ}{\mathrm{J}}
\newcommand{\rmk}{\mathrm{k}}
\newcommand{\rmK}{\mathrm{K}}
\newcommand{\rml}{\mathrm{l}}
\newcommand{\rmL}{\mathrm{L}}
\newcommand{\rmm}{\mathrm{m}}
\newcommand{\rmM}{\mathrm{M}}
\newcommand{\rmn}{\mathrm{n}}
\newcommand{\rmN}{\mathrm{N}}
\newcommand{\rmo}{\mathrm{o}}
\newcommand{\rmO}{\mathrm{O}}
\newcommand{\rmp}{\mathrm{p}}
\newcommand{\rmP}{\mathrm{P}}
\newcommand{\rmq}{\mathrm{q}}
\newcommand{\rmQ}{\mathrm{Q}}
\newcommand{\rmr}{\mathrm{r}}
\newcommand{\rmR}{\mathrm{R}}
\newcommand{\rms}{\mathrm{s}}
\newcommand{\rmS}{\mathrm{S}}
\newcommand{\rmt}{\mathrm{t}}
\newcommand{\rmT}{\mathrm{T}}
\newcommand{\rmu}{\mathrm{u}}
\newcommand{\rmU}{\mathrm{U}}
\newcommand{\rmv}{\mathrm{v}}
\newcommand{\rmV}{\mathrm{V}}
\newcommand{\rmw}{\mathrm{w}}
\newcommand{\rmW}{\mathrm{W}}
\newcommand{\rmx}{\mathrm{x}}
\newcommand{\rmX}{\mathrm{X}}
\newcommand{\rmy}{\mathrm{y}}
\newcommand{\rmY}{\mathrm{Y}}
\newcommand{\rmz}{\mathrm{z}}
\newcommand{\rmZ}{\mathrm{Z}}


% Numbers bb font
\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}


% Mathfrak font
\newcommand{\frakA}{\mathfrak{A}}
\newcommand{\frakB}{\mathfrak{B}}
\newcommand{\frakC}{\mathfrak{C}}
\newcommand{\frakD}{\mathfrak{D}}
\newcommand{\frakE}{\mathfrak{E}}
\newcommand{\frakF}{\mathfrak{F}}
\newcommand{\frakG}{\mathfrak{G}}
\newcommand{\frakH}{\mathfrak{H}}
\newcommand{\frakI}{\mathfrak{I}}
\newcommand{\frakJ}{\mathfrak{J}}
\newcommand{\frakK}{\mathfrak{K}}
\newcommand{\frakL}{\mathfrak{L}}
\newcommand{\frakM}{\mathfrak{M}}
\newcommand{\frakN}{\mathfrak{N}}
\newcommand{\frakO}{\mathfrak{O}}
\newcommand{\frakP}{\mathfrak{P}}
\newcommand{\frakQ}{\mathfrak{Q}}
\newcommand{\frakR}{\mathfrak{R}}
\newcommand{\frakS}{\mathfrak{S}}
\newcommand{\frakT}{\mathfrak{T}}
\newcommand{\frakU}{\mathfrak{U}}
\newcommand{\frakV}{\mathfrak{V}}
\newcommand{\frakW}{\mathfrak{W}}
\newcommand{\frakX}{\mathfrak{X}}
\newcommand{\frakY}{\mathfrak{Y}}
\newcommand{\frakZ}{\mathfrak{Z}}


% Mathscr
\newcommand{\scA}{\mathscr{A}}
\newcommand{\scB}{\mathscr{B}}
\newcommand{\scC}{\mathscr{C}}
\newcommand{\scD}{\mathscr{D}}
\newcommand{\scE}{\mathscr{E}}
\newcommand{\scF}{\mathscr{F}}
\newcommand{\scG}{\mathscr{G}}
\newcommand{\scH}{\mathscr{H}}
\newcommand{\scI}{\mathscr{I}}
\newcommand{\scJ}{\mathscr{J}}
\newcommand{\scK}{\mathscr{K}}
\newcommand{\scL}{\mathscr{L}}
\newcommand{\scM}{\mathscr{M}}
\newcommand{\scN}{\mathscr{N}}
\newcommand{\scO}{\mathscr{O}}
\newcommand{\scP}{\mathscr{P}}
\newcommand{\scQ}{\mathscr{Q}}
\newcommand{\scR}{\mathscr{R}}
\newcommand{\scS}{\mathscr{S}}
\newcommand{\scT}{\mathscr{T}}
\newcommand{\scU}{\mathscr{U}}
\newcommand{\scV}{\mathscr{V}}
\newcommand{\scW}{\mathscr{W}}
\newcommand{\scX}{\mathscr{X}}
\newcommand{\scY}{\mathscr{Y}}
\newcommand{\scZ}{\mathscr{Z}}

% San serif font
\DeclareMathAlphabet{\mathbsf}{OT1}{cmss}{bx}{n}
\DeclareMathAlphabet{\mathssf}{OT1}{cmss}{m}{sl}% slanted sans serif
\newcommand{\rva}{\mathsf{a}}
\newcommand{\rvA}{\mathsf{A}}
\newcommand{\rvba}{\mathbsf{a}}
\newcommand{\rvbA}{\mathbsf{A}}
\newcommand{\rvb}{\mathsf{b}}
\newcommand{\rvB}{\mathsf{B}}
\newcommand{\rvbb}{\mathbsf{b}}
\newcommand{\rvbB}{\mathbsf{B}}
\newcommand{\rvc}{\mathsf{c}}
\newcommand{\rvC}{\mathsf{C}}
\newcommand{\rvbc}{\mathbsf{c}}
\newcommand{\rvbC}{\mathbsf{C}}
\newcommand{\rvd}{\mathsf{d}}
\newcommand{\rvD}{\mathsf{D}}
\newcommand{\rvbd}{\mathbsf{d}}
\newcommand{\rvbD}{\mathbsf{D}}
\newcommand{\rve}{\mathsf{e}}
\newcommand{\rvE}{\mathsf{E}}
\newcommand{\rvbe}{\mathbsf{e}}
\newcommand{\rvbE}{\mathbsf{E}}
\newcommand{\rvf}{\mathsf{f}}
\newcommand{\rvF}{\mathsf{F}}
\newcommand{\rvbf}{\mathbsf{f}}
\newcommand{\rvbF}{\mathbsf{F}}
\newcommand{\rvg}{\mathsf{g}}
\newcommand{\rvG}{\mathsf{G}}
\newcommand{\rvbg}{\mathbsf{g}}
\newcommand{\rvbG}{\mathbsf{G}}
\newcommand{\rvh}{\mathsf{h}}
\newcommand{\rvH}{\mathsf{H}}
\newcommand{\rvbh}{\mathbsf{h}}
\newcommand{\rvbH}{\mathbsf{H}}
\newcommand{\rvi}{\mathsf{i}}
\newcommand{\rvI}{\mathsf{I}}
\newcommand{\rvbi}{\mathbsf{i}}
\newcommand{\rvbI}{\mathbsf{I}}
\newcommand{\rvj}{\mathsf{j}}
\newcommand{\rvJ}{\mathsf{J}}
\newcommand{\rvbj}{\mathbsf{j}}
\newcommand{\rvbJ}{\mathbsf{J}}
\newcommand{\rvk}{\mathsf{k}}
\newcommand{\rvK}{\mathsf{K}}
\newcommand{\rvbk}{\mathbsf{k}}
\newcommand{\rvbK}{\mathbsf{K}}
\newcommand{\rvl}{\mathsf{l}}
\newcommand{\rvL}{\mathsf{L}}
\newcommand{\rvbl}{\mathbsf{l}}
\newcommand{\rvbL}{\mathbsf{L}}
\newcommand{\rvm}{\mathsf{m}}
\newcommand{\rvM}{\mathsf{M}}
\newcommand{\rvbm}{\mathbsf{m}}
\newcommand{\rvbM}{\mathbsf{M}}
\newcommand{\rvn}{\mathsf{n}}
\newcommand{\rvN}{\mathsf{N}}
\newcommand{\rvbn}{\mathbsf{n}}
\newcommand{\rvbN}{\mathbsf{N}}
\newcommand{\rvo}{\mathsf{o}}
\newcommand{\rvO}{\mathsf{O}}
\newcommand{\rvbo}{\mathbsf{o}}
\newcommand{\rvbO}{\mathbsf{O}}
\newcommand{\rvp}{\mathsf{p}}
\newcommand{\rvP}{\mathsf{P}}
\newcommand{\rvbp}{\mathbsf{p}}
\newcommand{\rvbP}{\mathbsf{P}}
\newcommand{\rvq}{\mathsf{q}}
\newcommand{\rvQ}{\mathsf{Q}}
\newcommand{\rvbq}{\mathbsf{q}}
\newcommand{\rvbQ}{\mathbsf{Q}}
\newcommand{\rvr}{\mathsf{r}}
\newcommand{\rvR}{\mathsf{R}}
\newcommand{\rvbr}{\mathbsf{r}}
\newcommand{\rvbR}{\mathbsf{R}}
\newcommand{\rvs}{\mathsf{s}}
\newcommand{\rvS}{\mathsf{S}}
\newcommand{\rvbs}{\mathbsf{s}}
\newcommand{\rvbS}{\mathbsf{S}}
\newcommand{\rvt}{\mathsf{t}}
\newcommand{\rvT}{\mathsf{T}}
\newcommand{\rvbt}{\mathbsf{t}}
\newcommand{\rvbT}{\mathbsf{T}}
\newcommand{\rvu}{\mathsf{u}}
\newcommand{\rvU}{\mathsf{U}}
\newcommand{\rvbu}{\mathbsf{u}}
\newcommand{\rvbU}{\mathbsf{U}}
\newcommand{\rvv}{\mathsf{v}}
\newcommand{\rvV}{\mathsf{V}}
\newcommand{\rvbv}{\mathbsf{v}}
\newcommand{\rvbV}{\mathbsf{V}}
\newcommand{\rvw}{\mathsf{w}}
\newcommand{\rvW}{\mathsf{W}}
\newcommand{\rvbw}{\mathbsf{w}}
\newcommand{\rvbW}{\mathbsf{W}}
\newcommand{\rvx}{\mathsf{x}}
\newcommand{\rvX}{\mathsf{X}}
\newcommand{\rvbx}{\mathbsf{x}}
\newcommand{\rvbX}{\mathbsf{X}}
\newcommand{\rvy}{\mathsf{y}}
\newcommand{\rvY}{\mathsf{Y}}
\newcommand{\rvby}{\mathbsf{y}}
\newcommand{\rvbY}{\mathbsf{Y}}
\newcommand{\rvz}{\mathsf{z}}
\newcommand{\rvZ}{\mathsf{Z}}
\newcommand{\rvbz}{\mathbsf{z}}
\newcommand{\rvbZ}{\mathbsf{Z}}

\newcommand{\rvTh}{\ssfTheta}
\newcommand{\svTh}{\Theta}
\newcommand{\rvbTh}{\bsfTheta}
\newcommand{\svbTh}{\boldsymbol{\Theta}}
\newcommand{\rvPh}{\ssfPhi}
\newcommand{\svPh}{\Phi}
\newcommand{\rvbPh}{\bsfPhi}
\newcommand{\svbPh}{\boldsymbol{\Phi}}

% define some useful uppercase Greek letters in regular and bold sf
\DeclareSymbolFont{bsfletters}{OT1}{cmss}{bx}{n}  
\DeclareSymbolFont{ssfletters}{OT1}{cmss}{m}{n}
\DeclareMathSymbol{\bsfGamma}{0}{bsfletters}{'000}
\DeclareMathSymbol{\ssfGamma}{0}{ssfletters}{'000}
\DeclareMathSymbol{\bsfDelta}{0}{bsfletters}{'001}
\DeclareMathSymbol{\ssfDelta}{0}{ssfletters}{'001}
\DeclareMathSymbol{\bsfTheta}{0}{bsfletters}{'002}
\DeclareMathSymbol{\ssfTheta}{0}{ssfletters}{'002}
\DeclareMathSymbol{\bsfLambda}{0}{bsfletters}{'003}
\DeclareMathSymbol{\ssfLambda}{0}{ssfletters}{'003}
\DeclareMathSymbol{\bsfXi}{0}{bsfletters}{'004}
\DeclareMathSymbol{\ssfXi}{0}{ssfletters}{'004}
\DeclareMathSymbol{\bsfPi}{0}{bsfletters}{'005}
\DeclareMathSymbol{\ssfPi}{0}{ssfletters}{'005}
\DeclareMathSymbol{\bsfSigma}{0}{bsfletters}{'006}
\DeclareMathSymbol{\ssfSigma}{0}{ssfletters}{'006}
\DeclareMathSymbol{\bsfUpsilon}{0}{bsfletters}{'007}
\DeclareMathSymbol{\ssfUpsilon}{0}{ssfletters}{'007}
\DeclareMathSymbol{\bsfPhi}{0}{bsfletters}{'010}
\DeclareMathSymbol{\ssfPhi}{0}{ssfletters}{'010}
\DeclareMathSymbol{\bsfPsi}{0}{bsfletters}{'011}
\DeclareMathSymbol{\ssfPsi}{0}{ssfletters}{'011}
\DeclareMathSymbol{\bsfOmega}{0}{bsfletters}{'012}
\DeclareMathSymbol{\ssfOmega}{0}{ssfletters}{'012}

% Hat and Tilde
\newcommand{\hata}{\widehat{a}}
\newcommand{\hatA}{\widehat{A}}
\newcommand{\tila}{\widetilde{a}}
\newcommand{\tilA}{\widetilde{A}}
\newcommand{\hatba}{\widehat{\ba}}
\newcommand{\hatbA}{\widehat{\bA}}
\newcommand{\tilba}{\widetilde{\ba}}
\newcommand{\tilbA}{\widetilde{\bA}}

\newcommand{\hatb}{\widehat{b}}
\newcommand{\hatB}{\widehat{B}}
\newcommand{\tilb}{\widetilde{b}}
\newcommand{\tilB}{\widetilde{B}}
\newcommand{\hatbb}{\widehat{\bb}}
\newcommand{\hatbB}{\widehat{\bB}}
\newcommand{\tilbb}{\widetilde{\bb}}
\newcommand{\tilbB}{\widetilde{\bB}}

\newcommand{\hatc}{\widehat{c}}
\newcommand{\hatC}{\widehat{C}}
\newcommand{\tilc}{\widetilde{c}}
\newcommand{\tilC}{\widetilde{C}}
\newcommand{\hatbc}{\widehat{\bc}}
\newcommand{\hatbC}{\widehat{\bC}}
\newcommand{\tilbc}{\widetilde{\bc}}
\newcommand{\tilbC}{\widetilde{\bC}}

\newcommand{\hatd}{\widehat{d}}
\newcommand{\hatD}{\widehat{D}}
\newcommand{\tild}{\widetilde{d}}
\newcommand{\tilD}{\widetilde{D}}
\newcommand{\hatbd}{\widehat{\bd}}
\newcommand{\hatbD}{\widehat{\bD}}
\newcommand{\tilbd}{\widetilde{\bd}}
\newcommand{\tilbD}{\widetilde{\bD}}

\newcommand{\hate}{\widehat{e}}
\newcommand{\hatE}{\widehat{E}}
\newcommand{\tile}{\widetilde{e}}
\newcommand{\tilE}{\widetilde{E}}
\newcommand{\hatbe}{\widehat{\be}}
\newcommand{\hatbE}{\widehat{\bE}}
\newcommand{\tilbe}{\widetilde{\be}}
\newcommand{\tilbE}{\widetilde{\bE}}

\newcommand{\hatf}{\widehat{f}}
\newcommand{\hatF}{\widehat{F}}
\newcommand{\tilf}{\widetilde{f}}
\newcommand{\tilF}{\widetilde{F}}
\newcommand{\hatbf}{\widehat{\boldf}}
\newcommand{\hatbF}{\widehat{\bF}}
\newcommand{\tilbf}{\widetilde{\boldf}}
\newcommand{\tilbF}{\widetilde{\bF}}

\newcommand{\hatg}{\widehat{g}}
\newcommand{\hatG}{\widehat{G}}
\newcommand{\tilg}{\widetilde{g}}
\newcommand{\tilG}{\widetilde{G}}
\newcommand{\hatbg}{\widehat{\bg}}
\newcommand{\hatbG}{\widehat{\bG}}
\newcommand{\tilbg}{\widetilde{\bg}}
\newcommand{\tilbG}{\widetilde{\bG}}

\newcommand{\hath}{\widehat{h}}
\newcommand{\hatH}{\widehat{H}}
\newcommand{\tilh}{\widetilde{h}}
\newcommand{\tilH}{\widetilde{H}}
\newcommand{\hatbh}{\widehat{\bh}}
\newcommand{\hatbH}{\widehat{\bH}}
\newcommand{\tilbh}{\widetilde{\bh}}
\newcommand{\tilbH}{\widetilde{\bH}}

\newcommand{\hati}{\widehat{i}}
\newcommand{\hatI}{\widehat{I}}
\newcommand{\tili}{\widetilde{i}}
\newcommand{\tilI}{\widetilde{I}}
\newcommand{\hatbi}{\widehat{\bi}}
\newcommand{\hatbI}{\widehat{\bI}}
\newcommand{\tilbi}{\widetilde{\bi}}
\newcommand{\tilbI}{\widetilde{\bI}}

\newcommand{\hatj}{\widehat{j}}
\newcommand{\hatJ}{\widehat{J}}
\newcommand{\tilj}{\widetilde{j}}
\newcommand{\tilJ}{\widetilde{J}}
\newcommand{\hatbj}{\widehat{\bj}}
\newcommand{\hatbJ}{\widehat{\bJ}}
\newcommand{\tilbj}{\widetilde{\bj}}
\newcommand{\tilbJ}{\widetilde{\bJ}}

\newcommand{\hatk}{\widehat{k}}
\newcommand{\hatK}{\widehat{K}}
\newcommand{\tilk}{\widetilde{k}}
\newcommand{\tilK}{\widetilde{K}}
\newcommand{\hatbk}{\widehat{\bk}}
\newcommand{\hatbK}{\widehat{\bK}}
\newcommand{\tilbk}{\widetilde{\bk}}
\newcommand{\tilbK}{\widetilde{\bK}}

\newcommand{\hatl}{\widehat{l}}
\newcommand{\hatL}{\widehat{L}}
\newcommand{\till}{\widetilde{l}}
\newcommand{\tilL}{\widetilde{L}}
\newcommand{\hatbl}{\widehat{\bl}}
\newcommand{\hatbL}{\widehat{\bL}}
\newcommand{\tilbl}{\widetilde{\bl}}
\newcommand{\tilbL}{\widetilde{\bL}}

\newcommand{\hatm}{\widehat{m}}
\newcommand{\hatM}{\widehat{M}}
\newcommand{\tilm}{\widetilde{m}}
\newcommand{\tilM}{\widetilde{M}}
\newcommand{\hatbm}{\widehat{\boldm}}
\newcommand{\hatbM}{\widehat{\bM}}
\newcommand{\tilbm}{\widetilde{\boldm}}
\newcommand{\tilbM}{\widetilde{\bM}}

\newcommand{\hatn}{\widehat{n}}
\newcommand{\hatN}{\widehat{N}}
\newcommand{\tiln}{\widetilde{n}}
\newcommand{\tilN}{\widetilde{N}}
\newcommand{\hatbn}{\widehat{\bn}}
\newcommand{\hatbN}{\widehat{\bN}}
\newcommand{\tilbn}{\widetilde{\bn}}
\newcommand{\tilbN}{\widetilde{\bN}}

\newcommand{\hato}{\widehat{o}}
\newcommand{\hatO}{\widehat{O}}
\newcommand{\tilo}{\widetilde{o}}
\newcommand{\tilO}{\widetilde{O}}
\newcommand{\hatbo}{\widehat{\bo}}
\newcommand{\hatbO}{\widehat{\bO}}
\newcommand{\tilbo}{\widetilde{\bo}}
\newcommand{\tilbO}{\widetilde{\bO}}

\newcommand{\hatp}{\widehat{p}}
\newcommand{\hatP}{\widehat{P}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\tilP}{\widetilde{P}}
\newcommand{\hatbp}{\widehat{\bp}}
\newcommand{\hatbP}{\widehat{\bP}}
\newcommand{\tilbp}{\widetilde{\bp}}
\newcommand{\tilbP}{\widetilde{\bP}}

\newcommand{\hatq}{\widehat{q}}
\newcommand{\hatQ}{\widehat{Q}}
\newcommand{\tilq}{\widetilde{q}}
\newcommand{\tilQ}{\widetilde{Q}}
\newcommand{\hatbq}{\widehat{\bq}}
\newcommand{\hatbQ}{\widehat{\bQ}}
\newcommand{\tilbq}{\widetilde{\bq}}
\newcommand{\tilbQ}{\widetilde{\bQ}}

\newcommand{\hatr}{\widehat{r}}
\newcommand{\hatR}{\widehat{R}}
\newcommand{\tilr}{\widetilde{r}}
\newcommand{\tilR}{\widetilde{R}}
\newcommand{\hatbr}{\widehat{\br}}
\newcommand{\hatbR}{\widehat{\bR}}
\newcommand{\tilbr}{\widetilde{\br}}
\newcommand{\tilbR}{\widetilde{\bR}}

\newcommand{\hats}{\widehat{s}}
\newcommand{\hatS}{\widehat{S}}
\newcommand{\tils}{\widetilde{s}}
\newcommand{\tilS}{\widetilde{S}}
\newcommand{\hatbs}{\widehat{\bs}}
\newcommand{\hatbS}{\widehat{\bS}}
\newcommand{\tilbs}{\widetilde{\bs}}
\newcommand{\tilbS}{\widetilde{\bS}}

\newcommand{\hatt}{\widehat{t}}
\newcommand{\hatT}{\widehat{T}}
\newcommand{\tilt}{\widetilde{t}}
\newcommand{\tilT}{\widetilde{T}}
\newcommand{\hatbt}{\widehat{\bt}}
\newcommand{\hatbT}{\widehat{\bT}}
\newcommand{\tilbt}{\widetilde{\bt}}
\newcommand{\tilbT}{\widetilde{\bT}}

\newcommand{\hatu}{\widehat{u}}
\newcommand{\hatU}{\widehat{U}}
\newcommand{\tilu}{\widetilde{u}}
\newcommand{\tilU}{\widetilde{U}}
\newcommand{\hatbu}{\widehat{\bu}}
\newcommand{\hatbU}{\widehat{\bU}}
\newcommand{\tilbu}{\widetilde{\bu}}
\newcommand{\tilbU}{\widetilde{\bU}}

\newcommand{\hatv}{\widehat{v}}
\newcommand{\hatV}{\widehat{V}}
\newcommand{\tilv}{\widetilde{v}}
\newcommand{\tilV}{\widetilde{V}}
\newcommand{\hatbv}{\widehat{\bv}}
\newcommand{\hatbV}{\widehat{\bV}}
\newcommand{\tilbv}{\widetilde{\bv}}
\newcommand{\tilbV}{\widetilde{\bV}}

\newcommand{\hatw}{\widehat{w}}
\newcommand{\hatW}{\widehat{W}}
\newcommand{\tilw}{\widetilde{w}}
\newcommand{\tilW}{\widetilde{W}}
\newcommand{\hatbw}{\widehat{\bw}}
\newcommand{\hatbW}{\widehat{\bW}}
\newcommand{\tilbw}{\widetilde{\bw}}
\newcommand{\tilbW}{\widetilde{\bW}}

\newcommand{\hatx}{\widehat{x}}
\newcommand{\hatX}{\widehat{X}}
\newcommand{\tilx}{\widetilde{x}}
\newcommand{\tilX}{\widetilde{X}}
\newcommand{\hatbx}{\widehat{\bx}}
\newcommand{\hatbX}{\widehat{\bX}}
\newcommand{\tilbx}{\widetilde{\bx}}
\newcommand{\tilbX}{\widetilde{\bX}}

\newcommand{\haty}{\widehat{y}}
\newcommand{\hatY}{\widehat{Y}}
\newcommand{\tily}{\widetilde{y}}
\newcommand{\tilY}{\widetilde{Y}}
\newcommand{\hatby}{\widehat{\by}}
\newcommand{\hatbY}{\widehat{\bY}}
\newcommand{\tilby}{\widetilde{\by}}
\newcommand{\tilbY}{\widetilde{\bY}}

\newcommand{\hatz}{\widehat{z}}
\newcommand{\hatZ}{\widehat{Z}}
\newcommand{\tilz}{\widetilde{z}}
\newcommand{\tilZ}{\widetilde{Z}}
\newcommand{\hatbz}{\widehat{\bz}}
\newcommand{\hatbZ}{\widehat{\bZ}}
\newcommand{\tilbz}{\widetilde{\bz}}
\newcommand{\tilbZ}{\widetilde{\bZ}}

\newcommand{\bara}{\overline{a}}
\newcommand{\barb}{\overline{b}}
\newcommand{\barc}{\overline{c}}
\newcommand{\bard}{\overline{d}}
\newcommand{\bare}{\overline{e}}
\newcommand{\barf}{\overline{f}}
\newcommand{\barg}{\overline{g}}
\newcommand{\barh}{\overline{h}}
\newcommand{\bari}{\overline{i}}
\newcommand{\barj}{\overline{j}}
\newcommand{\bark}{\overline{k}}
\newcommand{\barl}{\overline{l}}
\newcommand{\barm}{\overline{m}}
\newcommand{\barn}{\overline{n}}
\newcommand{\baro}{\overline{o}}
\newcommand{\barp}{\overline{p}}
\newcommand{\barq}{\overline{q}}
\newcommand{\barr}{\overline{r}}
\newcommand{\bars}{\overline{s}}
\newcommand{\bart}{\overline{t}}
\newcommand{\baru}{\overline{u}}
\newcommand{\barv}{\overline{v}}
\newcommand{\barw}{\overline{w}}
\newcommand{\barx}{\overline{x}}
\newcommand{\bary}{\overline{y}}
\newcommand{\barz}{\overline{z}}

\newcommand{\barA}{\overline{A}}
\newcommand{\barB}{\overline{B}}
\newcommand{\barC}{\overline{C}}
\newcommand{\barD}{\overline{D}}
\newcommand{\barE}{\overline{E}}
\newcommand{\barF}{\overline{F}}
\newcommand{\barG}{\overline{G}}
\newcommand{\barH}{\overline{H}}
\newcommand{\barI}{\overline{I}}
\newcommand{\barJ}{\overline{J}}
\newcommand{\barK}{\overline{K}}
\newcommand{\barL}{\overline{L}}
\newcommand{\barM}{\overline{M}}
\newcommand{\barN}{\overline{N}}
\newcommand{\barO}{\overline{O}}
\newcommand{\barP}{\overline{P}}
\newcommand{\barQ}{\overline{Q}}
\newcommand{\barR}{\overline{R}}
\newcommand{\barS}{\overline{S}}
\newcommand{\barT}{\overline{T}}
\newcommand{\barU}{\overline{U}}
\newcommand{\barV}{\overline{V}}
\newcommand{\barW}{\overline{W}}
\newcommand{\barX}{\overline{X}}
\newcommand{\barY}{\overline{Y}}
\newcommand{\barZ}{\overline{Z}}





% Bold greek
\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bdelta}{\bm{\delta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\veps}{\varepsilon}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\bmeta}{\bm{\eta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\brho}{\bm{\rho}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bSigma	}{\bm{\Sigma}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bOmega}{\bm{\Omega}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bTheta}{\bm{\Theta}}

\newcommand{\talpha}{\widetilde{\alpha}}
\newcommand{\tbeta}{\widetilde{\beta}}
\newcommand{\tgamma}{\widetilde{\gamma}}
\newcommand{\tdelta}{\widetilde{\delta}}
\newcommand{\ttheta}{\widetilde{\theta}}
\newcommand{\ttau}{\widetilde{\tau}}
\newcommand{\tpi}{\widetilde{\pi}}
\newcommand{\tepsilon}{\widetilde{\epsilon}}
\newcommand{\tvarepsilon}{\widetilde{\varepsilon}}
\newcommand{\tsigma}{\widetilde{\sigma}}
\newcommand{\tzeta}{\widetilde{\zeta}}
\newcommand{\tmeta}{\widetilde{\eta}}
\newcommand{\tkappa}{\widetilde{\kappa}}
\newcommand{\tchi}{\widetilde{\chi}}
\newcommand{\tphi}{\widetilde{\phi}}
\newcommand{\tpsi}{\widetilde{\psi}}
\newcommand{\tomega}{\widetilde{\omega}}
\newcommand{\txi}{\widetilde{\xi}}
\newcommand{\tlambda}{\widetilde{\lambda}}
\newcommand{\trho}{\widetilde{\rho}}
\newcommand{\tnu}{\widetilde{\nu}}

\newcommand{\tDelta}{\widetilde{\Delta}}

\newcommand{\halpha}{\widehat{\alpha}}
\newcommand{\hbeta}{\widehat{\beta}}
\newcommand{\hgamma}{\widehat{\gamma}}
\newcommand{\hdelta}{\widehat{\delta}}
\newcommand{\htheta}{\widehat{\theta}}
\newcommand{\htau}{\widehat{\tau}}
\newcommand{\hpi}{\widehat{\pi}}
\newcommand{\hepsilon}{\widehat{\epsilon}}
\newcommand{\hvarepsilon}{\widehat{\varepsilon}}
\newcommand{\hsigma}{\widehat{\sigma}}
\newcommand{\hzeta}{\widehat{\zeta}}
\newcommand{\hmeta}{\widehat{\eta}}
\newcommand{\hkappa}{\widehat{\kappa}}
\newcommand{\hchi}{\widehat{\chi}}
\newcommand{\hphi}{\widehat{\phi}}
\newcommand{\hpsi}{\widehat{\psi}}
\newcommand{\homega}{\widehat{\omega}}
\newcommand{\hxi}{\widehat{\xi}}
\newcommand{\hlambda}{\widehat{\lambda}}
\newcommand{\hrho}{\widehat{\rho}}

% Define underlined letters
\newcommand{\ua}{\underline{a}}
\newcommand{\uA}{\underline{A}}
\newcommand{\ub}{\underline{b}}
\newcommand{\uB}{\underline{B}}
\newcommand{\uc}{\underline{c}}
\newcommand{\uC}{\underline{C}}
\newcommand{\ud}{\underline{d}}
\newcommand{\uD}{\underline{D}}
\newcommand{\ue}{\underline{e}}
\newcommand{\uE}{\underline{E}}
\newcommand{\uf}{\underline{f}}
\newcommand{\uF}{\underline{F}}
\newcommand{\ug}{\underline{g}}
\newcommand{\uG}{\underline{G}}
\newcommand{\uh}{\underline{h}}
\newcommand{\uH}{\underline{H}}
\newcommand{\ui}{\underline{i}}
\newcommand{\uI}{\underline{I}}
\newcommand{\uj}{\underline{j}}
\newcommand{\uJ}{\underline{J}}
\newcommand{\uk}{\underline{k}}
\newcommand{\uK}{\underline{K}}
\newcommand{\ul}{\underline{l}}
\newcommand{\uL}{\underline{L}}
\newcommand{\um}{\underline{m}}
\newcommand{\uM}{\underline{M}}
\newcommand{\un}{\underline{n}}
\newcommand{\uN}{\underline{N}}
\newcommand{\uo}{\underline{o}}
\newcommand{\uO}{\underline{O}}
\newcommand{\up}{\underline{p}}
\newcommand{\uP}{\underline{P}}
\newcommand{\uq}{\underline{q}}
\newcommand{\uQ}{\underline{Q}}
\newcommand{\ur}{\underline{r}}
\newcommand{\uR}{\underline{R}}
\newcommand{\us}{\underline{s}}
\newcommand{\uS}{\underline{S}}
\newcommand{\ut}{\underline{t}}
\newcommand{\uT}{\underline{T}}
\newcommand{\uu}{\underline{u}}
\newcommand{\uU}{\underline{U}}
\newcommand{\uv}{\underline{v}}
\newcommand{\uV}{\underline{V}}
\newcommand{\uw}{\underline{w}}
\newcommand{\uW}{\underline{W}}
\newcommand{\ux}{\underline{x}}
\newcommand{\uX}{\underline{X}}
\newcommand{\uy}{\underline{y}}
\newcommand{\uY}{\underline{Y}}
\newcommand{\uz}{\underline{z}}
\newcommand{\uZ}{\underline{Z}}


% functional dot

\def\fndot{\, \cdot \,}
\def\fndia{\, \diamond \,}
\def\fnstar{\, \star \,}

% exponential

\newcommand{\eexp}[1]{e^{#1}}

% iid

\newcommand{\iid}{i.i.d.\ }

% convergence

\newcommand{\convp}{\stackrel{\mathrm{p}}{\longrightarrow}}
\newcommand{\convwpone}{\stackrel{\mathrm{w.p.1}}{\longrightarrow}}
\newcommand{\convas}{\xrightarrow{\mathrm{a.s.}}}
\newcommand{\convd}{\stackrel{\mathrm{d}}{\longrightarrow}}
\newcommand{\convD}{\stackrel{\mathrm{D}}{\longrightarrow}}

\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}
\newcommand{\lrangle}[2]{\left\langle{#1},{#2}\right\rangle}


\newcommand{\dotleq}{\stackrel{.}{\leq}}
\newcommand{\dotlt}{\stackrel{.}{<}}
\newcommand{\dotgeq}{\stackrel{.}{\geq}}
\newcommand{\dotgt}{\stackrel{.}{>}}
\newcommand{\dotdoteq}{\stackrel{\,..}{=}}
% Inequalities
\newcommand{\eqa}{\stackrel{(a)}{=}}
\newcommand{\eqb}{\stackrel{(b)}{=}}
\newcommand{\eqc}{\stackrel{(c)}{=}}
\newcommand{\eqd}{\stackrel{(d)}{=}}
\newcommand{\eqe}{\stackrel{(e)}{=}}
\newcommand{\eqf}{\stackrel{(f)}{=}}
\newcommand{\eqg}{\stackrel{(g)}{=}}
\newcommand{\eqh}{\stackrel{(h)}{=}}
\newcommand{\lea}{\stackrel{(a)}{\le}}
\newcommand{\leb}{\stackrel{(b)}{\le}}
\newcommand{\lec}{\stackrel{(c)}{\le}}
\newcommand{\led}{\stackrel{(d)}{\le}}
\newcommand{\lee}{\stackrel{(e)}{\le}}
\newcommand{\lef}{\stackrel{(f)}{\le}}
\newcommand{\leg}{\stackrel{(g)}{\le}}
\newcommand{\leh}{\stackrel{(h)}{\le}}
\newcommand{\gea}{\stackrel{(a)}{\ge}}
\newcommand{\geb}{\stackrel{(b)}{\ge}}
\newcommand{\gec}{\stackrel{(c)}{\ge}}
\newcommand{\ged}{\stackrel{(d)}{\ge}}
\newcommand{\gee}{\stackrel{(e)}{\ge}}
\newcommand{\gef}{\stackrel{(f)}{\ge}}
\newcommand{\geg}{\stackrel{(g)}{\ge}}
\newcommand{\geh}{\stackrel{(h)}{\ge}}
 
\newcommand{\Pen}{P_{\mathrm{e}}^{(n)}}
\newcommand{\Penone}{P_{\mathrm{e}, 1}^{(n)}}
\newcommand{\Pentwo}{P_{\mathrm{e}, 2}^{(n)}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator{\minimize}{minimize}
\DeclareMathOperator{\maximize}{maximize}
%\DeclareMathOperator{\st}{subject\,\,to}
\DeclareMathOperator{\st}{s.t.\;}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\cum}{cum}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\var}{\mathsf{Var}}
\DeclareMathOperator{\Vol}{Vol}
\DeclareMathOperator{\cov}{\mathsf{Cov}}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\vect}{vec}
\newcommand{\Hb}{H_{\mathrm{b}}}%binary entropy
\newcommand{\Ber}{\mathrm{Bern}}
\DeclareMathOperator*{\lms}{l.i.m.\,}
\newcommand{\varop}[1]{\var\left[{#1}\right]}
\newcommand{\covop}[2]{\cov\left({#1},{#2}\right)} 
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}

\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern5mu{#1#2}}}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
 

\newtheorem{theorem}{Theorem}[section]
%\newtheorem{theorem}{Theorem}[within]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{example}{Example}
\newtheorem{exercise}{Exercise}

\newtheorem{fact}{Fact}[section]

\theoremstyle{definition}
\newtheorem{definition}{Definition} [section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}

%\theoremstyle{remark}
%\newtheorem*{psketch}{Proof Sketch}
\newenvironment{psketch}{\noindent{\em Proof Sketch.}\hspace*{1em}}{\qed\bigskip\\}

\renewcommand\qedsymbol{$\square$}

%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{{\hfill$\square$}\end{trivlist}}
%\newenvironment{psketch}[1][Proof Sketch]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{{\hfill$\square$}\end{trivlist}}
%\newenvironment{definition}[1][Definition]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{example}[1][Example]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{remark}[1][Remark]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
%\newenvironment{assump}[1][Assumption]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\newcommand{\qed}{\hfill$\square$}
\newcommand{\qednew}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}

